DnLUT: Ultra-Efficient Color Image Denoising via Channel-Aware Lookup Tables

While deep neural networks have revolutionized image denoising capabilities, their deployment on edge devices remains challenging due to substantial computational and memory requirements. To this end, we present DnLUT, an ultra-efficient lookup table-based framework that achieves high-quality color image denoising with minimal resource consumption. Our key innovation lies in two complementary components: a Pairwise Channel Mixer (PCM) that effectively captures inter-channel correlations and spatial dependencies in parallel, and a novel L-shaped convolution design that maximizes receptive field coverage while minimizing storage overhead. By converting these components into optimized lookup tables post-training, DnLUT achieves remarkable efficiency - requiring only 500KB storage and 0.1% energy consumption compared to its CNN contestant DnCNN, while delivering 20X faster inference. Extensive experiments demonstrate that DnLUT outperforms all existing LUT-based methods by over 1dB in PSNR, establishing a new state-of-the-art in resource-efficient color image denoising. The project is available at https://github.com/Stephen0808/DnLUT.

==> sec/0_abstract_bak.tex <==
\begin{abstract}
\label{abs}
Despite the surge of deep neural networks ushering in an era of unprecedented image denoising capabilities, models with multi-layer networks have struggled to apply on edge devices such as low-end smartphones, monitors, and televisions due to their high storage memory and computational resource requirements. To address this challenge, we propose an efficient color image denoising method based on lookup tables (LUTs). In this task, we must consider both channel and spatial information in parallel while maintaining a comparably small storage size. During training, we compose pairwise channels from RGB into three groups to extract channel correlation. To further enlarge the spatial receptive field and compress the LUT size, we introduce a novel L-shaped convolution to fully exploit pixel information. After training, the convolutions will be converted into LUTs for efficient inference. The overall LUT size is around 500KB, yet our method outperforms all LUT-based methods by over 1dB PSNR improvement, with $0.1\%$ energy cost and $20\times$ speedup of DnCNN.
\end{abstract}

==> sec/1_intro_bak.tex <==
\section{Introduction}
\label{sec:intro}
Color images are ubiquitous in photography, social media, and scientific signal processing. Compared to grayscale images, color images are more susceptible to noise during acquisition, storage, and transmission due to their threefold size. Additionally, human perception is more sensitive to color than luminance, making artifacts in color images more readily apparent. 

In recent years, with the rapid development of deep learning, methods based on deep neural networks (DNN) have made impressive progress in color image denoising\cite{zhang2017beyond, liang2021swinir, zamir2022restormer, chen2021pre, zhang2023kbnet}. In general, the common feature of a series of state-of-the-art models is that they come with numerous convolutional layers or transformer blocks appealing to several multiplication operations. However, the high computational complexity and memory consumption of these models hinder further application to edge devices. Specifically, most edge devices lack parallel computing devices, such as graphic processing units (GPUs) or tensor processing units (TPUs). Therefore, despite the surge in deep neural networks, significant questions remain about their practical application.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/teaser.pdf}
    \caption{Model comparison in terms of PSNR (dB), runtime,
and storage. The PSNR and runtime are calculated on the
CBSD68 with the Gaussian noise level $\sigma = 25$ based on the Qualcomm Snapdragon 8 Gen2. The proposed method outperforms the state-of-the-art LUT-based methods with higher cPSNR, lower storage size, and less runtime. The main module, PCM, could be a versatile plug-in module to enhance the performance by over 1dB.
}
    \label{fig:enter-label}
\end{figure}

To answer this question, several recent works have harnessed lookup tables (LUTs) for efficient image super-resolution. A LUT is an array that replaces runtime computation with a simpler array indexing operation, known as direct addressing. These works first devise several elegant modules for training. After training, they traverse all possible input value combinations to form complete LUTs. During inference, LUTs are used to index the results without requiring time-consuming and energy-cost computation. These methods leverage the capabilities of DNNs while freeing deployment from hardware constraints. So, low-end devices with limited caches could also apply this kind of technique for image enhancement. However, the size of a single LUT grows exponentially with the increase in its indexing capacity. Hence, 4D LUT (using 4 pixel values for indexing) is empirically recognized as the trade-off of storage and performance. Specifically, $2\times2$ convolutional kernel is adapted to each channel seperately\cite{jo2021practical, li2022mulut, liu2023reconstructed, li2024look}, which is then converted into a 4D LUT, referred to as a spatial-wise LUT for single-channel processing. However, the cached input-output pairs of lookup tables built from a single channel remain questionable for color image denoising, as noise typically invades all RGB channels, making channel correlation crucial for the denoising process.
A simple approach  to address this issue is to use a $1 \times 1$ convolutional kernel with the depth of 3 to extract RGB channel information and then convert it to a 3D channel-wise LUT\cite{li2024toward, yang2024taming}. However, mechanically combining the spatial-wise LUT and channel-wise LUT still yields inferior results. Naively extracting color information disrupts the noise distribution, making it difficult for subsequent spatial convolutions to model the degradation. Another approach is to employ the $H\times W \times 3$ kernel ($H>1, W>1$), similar to a standard convolution kernel, to construct the network. However, as mentioned before, the large receptive field (RF) can lead to an exponential increase in the storage space required for the LUT.

To this end, we propose a color image denoising model based on lookup tables (DnLUT) that is capable of modeling spatial and channel correlations while being applicable to edge device applications, with a focus on small storage space, low power consumption, and fast inference speed. First, we introduce a Pairwise Channel Mixer (PCM) to simultaneously fuse spatial and channel information. In this module, we first sample two channels from RGB to form three pairwise channel combinations: RG, RB, and GB. These combinations are processed in parallel across three branches. Next, we adapt a convolutional kernel with a spatial dimension of $1\times2$ and a depth of 2 to each pairwise channel in parallel at the first layer. The RF size of the remaining layers is set to $1 \times 1$ to keep the number of involved pixels small.This module can be seamlessly converted into three 4D LUTs after training. Not only does it leverage the strong generalization capabilities of deep neural networks, but it also benefits from the efficiency of lookup operations. Additionally, it can serve as a plug-in module for existing LUT-based methods, improving performance by about 1dB.

After taking the channel correlation into account, as discussed in \cite{li2022mulut, li2024look}, there is still a need to enlarge the spatial receptive field. SR-LUT\cite{jo2021practical} proposed a rotation ensemble training strategy to expand the RF size. However, stacking several spatial-wise LUTs results in significant storage burdens. We find that, except for the pivot pixel, a portion of pixels are repeatedly involved in the lookup operation, or overlapping pixels in the rotations. Repeatedly using the pixels will not bring improvement but will increase the inference burden. Therefore, we propose a novel L-shaped convolutional kernel including 2 other pixels by each rotation, fully making use of this strategy without overlapping pixels. A 4-rotation ensemble with 0, 90, 180, and 270 degrees covers a total of 9 ($3\times3$) pixels, but what's remarkable is that it compresses the 4D LUT to a 3D LUT, allowing for an enlarged RF size with minimal storage burden.

Extensive experiments demonstrate a clear advantage of our proposed DnLUT over state-of-the-art LUT methods. On four standard Gaussian denoising benchmarks, DnLUT achieves up to 1.3dB cPSNR improvement compared to SPFLUT\cite{li2024look}. For real-world color image denoising, DnLUT outperforms CBM3D\cite{dabov2007color} by nearly 5dB. Meanwhile, DnLUT preserves the efficiency of LUT-based methods. For example, the energy cost is about $0.1\%$ of DNCNN and require only 500KB of storage space.

\begin{itemize}
\item We propose a pairwise channel mixer (PCM) to fully exploit channel and spatial correlations. This module could serve as a plug-in module for existing LUT-based methods, bringing over 1dB cPSNR improvement.
\item We propose an L-shaped convolution module for compressing the LUT size. This module could be seamlessly converted to 3D LUT, saving $\times 17$ storage occupation during inference while maintaining the same RF size compared to 4D LUT. 
\item DnLUT outpeforms all the LUT-based methods by over 1dB on synthetic datasets and 0.5dB on real-world datasets. It only need $0.1\%$ energy cost of DnCNN and 500KB storage occupation during inference.
\end{itemize}

==> sec/2_related_bak.tex <==
\section{Related works}
\label{sec:related}

\subsection{Color Image denoising}
It is well-known that in color images, the RGB channels are highly correlated with each other\cite{dai2013multichannel}. Processing each channel separately often yields inferior performance compared to processing the color channels jointly\cite{mairal2007sparse}. Given this inherent nature, previous research has explored leveraging color correlation to enhance the denoised image quality.
One notable approach is CBM3D\cite{dabov2007color}, which transforms the RGB image into a luminance-chrominance space (\eg $YC_bC_r$). It performs grouping using BM3D\cite{dabov2007image} only once for the luminance channel (Y) and reuses the same grouping when applying collaborative filtering on the chrominance channels $U$ and $V$. \cite{lefkimmiatis2017non} adopt a similar grouping strategy but introduce a radial basis function mixture to handle color correlations separately. Building on the prior work of WNNM\cite{gu2014weighted}, MC-WNNM\cite{xu2017multi} introduces a weight matrix to balance the data fidelity of the three channels, considering their different noise statistics. 
In the last decade, DnCNN\cite{zhang2017beyond} heralded the advent of deep neural networks for color image denoising. Most subsequent works, such as \cite{zamir2021multi, zamir2022restormer, liang2021swinir, chen2021pre, zhang2023kbnet}, have involved all three RGB channels as input and processed them using convolution layers or transformer blocks. By treating the RGB channels as a whole, these models achieve high performance but require substantial computational resources and memory, posing a significant challenge for the development of deep learning in image processing.

\subsection{Replacing CNN with LUT}
How to extend the powerful capabilities of deep neural networks to edge devices has always been a huge challenge. Recently, several works have delved into converting neural networks into LUTs to bypass computation. Motivated by the color LUT in ISP, \cite{zeng2020learning} proposes to learn a series of basis LUTs with a weight prediction network to form a color LUT for mapping the input images to enhanced results. Following this work, \cite{yang2024taming} proposes an efficient enhancer based on channel-wise LUT with lower cost. However, the channel-wise LUT only involved one pixel from each channel, which is incapable of denoising. ~\cite{jo2021practical} first converts the CNN with a limited receptive field into spatial-wise LUTs for super-resolution. In such a paradigm, the network receives restricted pixels (e.g., $2\times2$) and predicts corresponding super-resolution pixels during training. The CNN is then transferred into a LUT by traversing all possible combinations of input values in the receptive field. During inference, the model uses the coordinate index to retrieve the corresponding output pixels cached in a LUT cell. The subsequent work~\cite{ma2022learning, li2022mulut, liu2023reconstructed} adopts serial LUTs for enlarging the receptive field and achieves a large PSNR improvement. To fully exploit the spatial pixels while avoiding exponential blow-up of the LUT size, these methods only build independent LUTs for a single input channel, i.e., treating the RGB channels unanimously. However, unlike super-resolution, which focuses on restoring high-frequency details by utilizing spatial information, color image denoising requires preserving spatial and channel information due to noise distribution. Hence, the aforementioned channel-wise or spatial-wise LUTs are not viable for color image denoising.


==> sec/3_method_bak.tex <==
\section{Method}
\subsection{Preliminary}
The LUT-based paradigm for image restoration is proposed by SR-LUT\cite{jo2021practical}. It adopts restricted receptive field for training a network(\eg $2\times2$). After that, the output values of the
trained network are cached into a LUT by traversing all possible pixel value combinations as input. During inference, the input patch with $2\times2$ shape is converted to the index of a 4D LUT for accessing the corresponding output value. Considering the huge storage, the 4D index is uniformly
subsampled with a sampling interval. Simultaneously, the rotation ensemble strategy is applied to rotate a small $2 \times 2$ input patch 4 times, contributing on a $3\times 3$ ensembled receptive field. Limited by the small receptive field, several works focus on enlarging the number of involved pixels by adapting multiple LUTs\cite{li2022mulut, ma2022learning, li2024look}, shift aggregations\cite{ma2022learning}, designing multiple kernel patterns\cite{li2022mulut, liu2023reconstructed, huang2023hundred}, etc.

In this paper, we delve into the LUT-based color image denoising, which is the most common task for edge devices.

% \subsection{Dilemma}
One common feature of these LUT-based works is that the kernel depth is set to 1. For color images, each RGB channel seperately looks up the cached output value without any interaction. This pipeline ignores the correlation of RGB channels, as well as the spatial-channel-wise degradation distribution in color image denoising. A naive way to handle the dilemma is to design kernel patterns like the vanilla convolution kernel. However, the LUT size increases exponentially with the index dimension, hindering the application of depth-wise kernels, as well as further application to color image processing tasks. For example, if we want to use the kernel with the shape of $2\times2$ and depth of 3, the LUT size is about 582 TB even with subsampling for compressing the size. As a result, the unaffordable storage seems to herald a verdict for LUT-based methods: \textbf{when aiming to capture more spatial information, we have to sacrifice the richness of channel information.} On the other hand, since adapting 4D spatial-wise LUTs leads to better performance, it always need multiple LUTs, similar to stacked convolution layers, which leads to a storage burden, especially when accessing the LUTs in the L1 cache.

\begin{table}[th]
% \vspace{-1em}
    \centering
    \caption{LUT size versus receptive field (RF) and channel numbers. * means subsampled LUT size}
    \begin{tabular}
    % {cccc}
    {p{10mm}<{\centering} p{10mm}<{\centering} p{15mm}<{\centering} p{25mm}<{\centering}}
        \toprule[1.1pt]
        RF& Depth &LUT Dim.& LUT Size*\\
        \hline
        $1\times1$ & 1 & 1D &17 B\\
        $1\times1$& 3& 3D &4.9 KB\\
        $2\times2$ & 1 & 4D &83.5 KB\\
        $1\times2$ & 3 & 6D &24.1 MB\\
        $2\times2$ & 3 & 12D & 582.6 TB\\
        $k\times k$ & c & $k \times k \times c$D & $(2^{4}+1)^{k \times k \times C}$ B\\
        \bottomrule[1.1pt]
    \end{tabular}
    % \vspace{-3em}
    \label{tab:tradeoff}
\end{table}

\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/pipeline.pdf}
    \caption{(a) Pipeline of DnNet. DnNet is composed of pairwise channel mixers and L-shaped convolutions. The multi-scale fusion is applied for enlarging the receptive field. We flatten the channel dimension for processing three channels in parallel since L-shaped only involved spatial pixels and then unfold back for inputting to PCM. (b) Pixels are rotated 4 times and then rotated back when processed by the DnNet. 4 outputs are ensembled through average. (c) After training, the corresponding outputs are traversed by all possible inputs through all the modules in DnNet. The outputs are cached in 3D or 4D LUTs for inference.(d) During inference, the input pixels are indexed by multiple LUTs. Each LUT indexes are generated by the cached outputs in prior LUTs, except for the final LUT, which generates the denoised pixel values. }
    \label{fig:enter-label}
\end{figure*}

\subsection{Overview}
Based on the observation, we try to handle these two dilemmas by proposing two modules: 1) a pairwise channel mixer that inherits the efficiency of 4D LUT but can model the spatial-channel correlations; 2) a novel L-shaped kernel with a nature of rotation non-overlapping, which can be converted to 3D LUT with the same receptive field like 4D LUT.

Our proposed color image denoising LUT framework, DnLUT, enhances the original spatial-wise LUT to achieve a better performance with two main modules: the pariwsie channel mixer is used to build the channel-spatial correlations and the L-shaped kernel helps the network see more pixels with minimal cost. We cascaded PCM with L-shaped convolution in two stages. In the first stage, inspired by previous works\cite{li2024look}, DnLUT predicts multiple-channel features from LUT groups and the multi-scale features are concatenated to the fusion module. The second one is the combination of the proposed two modules. Note that all the modules could be converted to 4D and 3D LUT during inference.

\subsection{Pairwise Channel Mixer}
Designing kernel patterns for LUT-based methods is a challenging task. Figure \ref{fig:diff_wise} illustrates the categories of various kernel patterns. Specifically, previous works have primarily focused on proposing single-dimension kernels, constrained by the limited LUT index dimension. There are two main disadvantages to applying these kernels for color image denoising. On the one hand, spatial-wise kernels concentrate on extracting spatial information, neglecting channel correlation, which results in color distortion and suboptimal noise modeling. On the other hand, channel-wise kernels establish a strong connection among RGB channels, but they ignore spatial information, leading to the persistence of significant artifacts. A straightforward approach to capturing both spatial and channel information is to combine these two kernels into a cascade network. However, this combination can't process both channel and spatial information synchronously and often yields inferior results due to the difficulty in modeling the noise distribution.

To address this challenge, we introduce the Pairwise Channel Mixer (PCM) for color image denoising. Initially, the RGB channels are separated by combining two different channels to create three pairwise channel outputs. These pairwise channels are then processed by a kernel with the shape of $1\times2$ and a depth of 2 from the first layer. Following this, multiple $1\times1$ convolution layers are cascaded to form a module. In this configuration, each convolution operation takes four pixel values as input and produces one channel as output. After training, this module can be seamlessly converted into a 4D LUT. The cached LUTs, \eg, $LUT_{RG}, LUT_{GB}$, and $LUT_{GR}$, are retrieved in parallel, after which their predictions are concatenated. Thus, for anchor
$(I_{R}, I_{G}, I_{B})$, the corresponding output values $(V_{R}, V_{G}, V_{B})$ are obtained by

\begin{equation}
\begin{aligned}
    (V_{R}, V_{G}, V_{B}) &= \text{Cat}(LUT_{RG}[I_{R,0,0}][I_{R,0,1}][I_{G,0,0}][I_{G,0,1}], \\
                           &\quad \quad \quad LUT_{GB}[I_{G,0,0}][I_{G,0,1}][I_{B,0,0}][I_{B,0,1}], \\
                           &\quad \quad \quad LUT_{BR}[I_{B,0,0}][I_{B,0,1}][I_{R,0,0}][I_{R,0,1}]),
\end{aligned}%
\end{equation}%
where C, H, W of each $I_{C,H,W}$ denotes channel, height, and width index. The PCM leverages the strengths of both spatial and channel-wise information processing. By combining two channels, the method captures inter-channel correlations, which are crucial for maintaining color fidelity during denoising. The $1\times2$ kernel ensures that spatial relationships are preserved, while the cascaded $1\times1$ convolutions refine the feature representations.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/different_wise.pdf}
    \caption{Different kernel pattern for LUT-based methods. The dark cube indicates the rotation point, and the medium dark indicates the involved pixel position in a rotation.}
    \label{fig:diff_wise}
\end{figure}

\subsection{Rotation Non-overlapping Kernel}
The rotation ensemble strategy plays a vital role in LUT-based methods. 4 rotational ensembles with 0, 90, 180, and 270 degrees help the asymmetric convolution kernels to cover a larger symmetric area. By weighted summing the outputs from the four rotations to generate the final result, the model achieves better performance without escalating the LUT index dimension. As shown in Fig.~\ref{fig:non-overlapping}, both SR-LUT and MuLUT utilize the strategy to enlarge the receptive field to $3\times 3$ and $5 \times 5$. 
However, this kernel design has two significant drawbacks. Firstly, nearly half of the pixel values within the receptive field are utilized at least twice during the lookup operation, as shown in the tables in Fig.~\ref{fig:non-overlapping}. This redundancy in the repeated usage of pixel values indicates a substantial inefficiency in the kernel patterns. Secondly, when stacking these kernels to form multiple LUTs for enlarging the receptive field, the resulting 4D LUT incurs a non-trivial storage cost.
To address these issues, we propose a novel and elegant kernel with an "L" shape. During each rotation, this kernel involves other two (except the center pixel) pixel values without any overlapping, contributing to the output with each surrounding pixel being used only once. This L-shaped kernel maximizes the utilization of pixel values within the receptive field. More importantly, it allows the kernel to be converted into a 3D LUT instead of a 4D LUT, thereby reducing storage requirements by at least an order of magnitude. 

\subsection{PCM Plug-in Module}
To further prove the effectiveness of the pairwise channel mixer module, we design the PCM as a plug-in module to be easily incorporated into any LUT-based methods for perceiving the spatial-channel correlations. Our PCM-Pulgin module can be easily put ahead of other LUT methods without any base structure change. This module gives these methods the ability of capturing channel-spatial correlations, leading to a large performance elevation. Compared to the state-of-the-art LUT methods, SPFLUT, it brings $\%12$ runtime and $\%8$ storage cost, but enhance the performance over 1dB.





\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figure/non-overlapping.pdf}
    \caption{Three different spatial-wise kernels. The left pattern in each subfigure indicates the kernel pattern, while the right table denotes the lookup times when retrieving the output value.}
    \label{fig:non-overlapping}
\end{figure}


==> sec/4_experiment_bak.tex <==
\section{Experiments}


\begin{table*}[htp]
    \centering
    \caption{Quantitative comparison on Gaussian color image denoising benchmark. The table presents cPSNR(dB) values.}
    \resizebox{2\columnwidth}{!}{
    \setlength{\tabcolsep}{1.5mm}{
    \begin{tabular}{ccccccccccccccccc}
        \toprule[1.1pt]
        \multirow{2}{*}{Method} &Storage & \multicolumn{3}{c}{CBSD68} & \multicolumn{3}{c}{Kodak24}&   \multicolumn{3}{c}{Urban100} &\multicolumn{3}{c}{McMaster}\\
        \cmidrule(r){3-5}
        \cmidrule(r){6-8}
        \cmidrule(r){9-11}
        \cmidrule(r){12-14}
        &(MB) & $\sigma = 15$ & $\sigma = 25$ &$\sigma = 50$ &$\sigma = 15$ & $\sigma = 25$ &$\sigma = 50$ &$\sigma = 15$ & $\sigma = 25$ &$\sigma = 50$ &$\sigma = 15$ & $\sigma = 25$ &$\sigma = 50$ \\
        \hline
        SR-LUT\cite{jo2021practical} &0.080 &29.76 & 26.71& 22.41&30.35 & 27.16& 22.65& 29.38 & 26.04& 21.60&31.18 & 28.01&23.35\\
         MuLUT\cite{li2022mulut} & 0.478 &30.52 & 28.11& 24.85& 31.31& 29.02& 25.28 & 30.25& 27.67& 23.75& 32.28& 29.88& 26.36\\
         RC-LUT\cite{liu2023reconstructed} & 0.239 &30.68 & 28.12&25.04 & 31.57 & 29.07& 25.89&30.33 & 27.80 & 23.86& 32.51&29.89&26.50\\
         % HKLUT &  &\\
         SPF-LUT\cite{li2024look} & 1.195 & 30.97 & 28.56 &25.33 & 31.86 & 29.58 &26.26 & 30.89 & 28.26& 24.22 &31.77 & 30.44 & 26.91\\
         DnLUT(Ours) & 0.516 & 32.41 & 29.88 & 26.03 &  33.02 & 30.24 & 26.74 & 32.12 & 28.87 & 25.01 & 32.88 & 30.44& 27.12\\ 
\midrule
         CBM3D\cite{dabov2007color} & - &33.52 & 30.71 & 27.38 & 34.28 & 31.68 & 29.02 &33.93 & 31.36&27.93&34.06 & 31.66 & 28.51 \\
         MC-WNNM\cite{xu2017multi} & - &31.98 & 29.32 & 26.98 & 33.23 & 30.89 & 28.67 & 30.23 & 29.23& 27.00& 31.23 & 30.20 & 27.55\\
\midrule
         DnCNN\cite{zhang2017beyond} & 2.239 &33.90 & 31.24 & 27.95 & 34.60 & 32.14 & 28.96& 32.98 & 30.81 & 27.59 & 33.45 & 31.52 & 28.62 \\
         % FFDNet \\
         SwinIR\cite{liang2021swinir} &45.499 & 34.42 & 31.78 & 28.56 & 35.34 & 32.89 & 29.79 & 35.61 & 33.20 & 30.22 & 35.13 & 32.90 & 29.82\\
        \bottomrule[1.1pt]
        % \vspace{-1.0em}
        
    \end{tabular}}
    }
    \label{tab:benchmark}
\end{table*}




\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/Gaussian.pdf}
    \caption{Qualitative comparison on synthetic datasets.}
    \label{fig:Gua}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/SIDD.pdf}
    \caption{Qualitative comparison on real-world datasets.}
    \label{fig:sidd}
\end{figure*}

\begin{table*}[htp]
    \centering
    \caption{Quantitative comparison on real-world color image denoising. The table presents cPSNR(dB) and SSIM values. Methods on DnD dataset are validated on the online platform. We could only get the PSNR rather than cPSNR.}
    \setlength{\tabcolsep}{1.5mm}{
    \resizebox{2\columnwidth}{!}{
    \begin{tabular}{cccccccccccccccc}
        \toprule[1.1pt]
        \textbf{Datasets} & Method & SR-LUT\cite{jo2021practical} & MuLUT\cite{li2022mulut} & RC-LUT\cite{liu2023reconstructed} & SPF-LUT\cite{li2024look} & DnLUT(Ours) & CBM3D\cite{dabov2007color} & MC-WNNM\cite{xu2017multi} & DnCNN\cite{zhang2017beyond} \\
        \hline
        \multirow{2}{*}{SIDD} & cPSNR &29.38 & 33.24 & 33.88 & 34.91 & 35.44 & 30.14 & 29.45 & 36.45 \\
         & SSIM & 0.634 & 0.830 & 0.839 & 0.865 & 0.875 & 0.702 & 0.682 & 0.900\\
         \hline
         \multirow{2}{*}{DnD} & PSNR$^{*}$ & 33.69&35.39 & 35.83& 36.22& 36.67 & 33.12& 32.34& 37.11\\
         
         & SSIM &0.839 & 0.887& 0.895&0.911 & 0.922 & 0.823 & 0.817& 0.932\\
        \bottomrule[1.1pt]
        % \vspace{-1.0em}
        
    \end{tabular}}
    }
    \label{tab:sidd}
\end{table*}



\begin{table*}[htp]
    \centering
    \caption{PCM can be easily incorporated to the existing LUT-based methods. It equips the model with the ability of capturing the channel correlations which  brings more than 1dB on the widely used benchmark. The noise level $\sigma$ of Gaussian noise is set to 25. The table presents cPSNR(dB) values.}
    \begin{tabular}{cccccc}
        \toprule[1.1pt]
        Method& CBSD68 & Kodak24 & Urban100 & McMaster & SIDD \\
        \hline
        SR-LUT\cite{jo2021practical} & 26.71 & 27.16 & 26.04 & 28.01 &29.38\\
        PCM+SR-LUT & 28.04\textcolor{red}{(+1.33)} & 28.55\textcolor{red}{(+1.39)} & 27.33\textcolor{red}{(+1.29)} & 28.78\textcolor{red}{(+0.77)} & 32.33\textcolor{red}{(+2.96)}\\
        MuLUT\cite{li2022mulut} & 28.11 & 29.01 & 27.67 & 29.88 & 33.24\\
        PCM+MuLUT & 29.17\textcolor{red}{(+1.05)} & 29.92\textcolor{red}{(+0.91)} & 28.74\textcolor{red}{(+1.07)} & 30.33\textcolor{red}{(+0.44)}& 34.33\textcolor{red}{(+1.09)}\\
        RC-LUT\cite{liu2023reconstructed} & 28.12 & 29.07 & 27.80 & 29.89 &33.88\\
        PCM+RC-LUT & 29.22\textcolor{red}{(+1.10)} & 30.09\textcolor{red}{(+1.02)} & 28.77\textcolor{red}{(+0.97)} & 30.54\textcolor{red}{(+0.65)}& 34.67\textcolor{red}{(+0.79)}\\
        SPF-LUT\cite{li2024look} & 28.56 & 29.58 & 28.26 & 30.44 & 34.91\\
        PCM+SPF-LUT & 29.72\textcolor{red}{(+1.16)} & 30.63\textcolor{red}{(+1.05)} & 29.43\textcolor{red}{(+1.17)}& 30.96\textcolor{red}{(+0.52)} & 35.56\textcolor{red}{(+0.65)}\\
        \bottomrule[1.1pt]
        \vspace{-1.0em}
    \end{tabular}
    \label{tab:pcm}
\end{table*}



\subsection{Implementation details}
We train DnLUT networks using the Adam optimizer with a cosine annealing learning rate schedule. The mean squared error (MSE) loss function is employed as the optimization target. For Gaussian denoising, the networks are trained for $2 \times 10^5$ iterations with a batch size of 12. In the case of real-world denoising, the batch size is increased to 32. Following the methodology of previous works \cite{jo2021practical, li2022mulut}, our LUTs are uniformly sampled at intervals of $2^4$. To mitigate indexing distortions, the final predictions are derived using 4D simplex interpolation and 3D tetrahedral interpolation. Additionally, we fine-tune the cached LUTs on the same training dataset for 2000 iterations using the LUT-aware fine-tuning strategy\cite{li2022mulut}.

\subsection{Gaussian Color Image denoising}
To validate the performance of our method, we follow the previous work \cite{zamir2022restormer} to train our model in the four datasets: DIV2K\cite{Agustsson_2017_CVPR_Workshops}, Flickr2K\cite{timofte2017ntire}, BSD400\cite{MartinFTM01}, and WaterlooED\cite{ma2016waterloo}, generated with the additive Gaussian noise over 3 noise levels ($\sigma \in \{15, 25, 50\}$). The methods are tested on four widely used color image datasets: CBSD68\cite{martin2001database}, Kodak24, Urban100\cite{huang2015single}, and McMaster\cite{zhang2011color} with the same Gaussian noise level.

\subsection{Real-world Color Image denoising}
For real-world color image denoising, we first train our method on the SIDD training datasets and conduct experiment on SIDD validation and DnD dataset to evaluate our method. The SIDD dataset is collected on indoor scenes captured by five smartphones at different noise levels. SIDD contains 320 image pairs for training and 1,280 for validation. DnD dataset is consisting of 50 high-resolution images with realistic image noise for evaluation.

\subsection{Quantitative results}
We employ two metrics, cPSNR and SSIM to assess the performance of the methods. We compare our method with the exsting LUT-based methods (SR-LUT\cite{jo2021practical}, MuLUT\cite{li2022mulut}, RC-LUT\cite{liu2023reconstructed}, and SPF-LUT\cite{li2024look}),  classical methods (CBM3D\cite{dabov2007color}, MC-WNNM(\cite{xu2017multi}), and the DNN-based mothods (DnCNN\cite{zhang2017beyond} and SwinIR\cite{liang2021swinir}). From the Tab.~\ref{tab:benchmark}, our method achieve best performance in the LUT-based category by surpassing the SPF-LUT over 1dB in the Gaussian color image denoising with only $17\%$ storage. From the Tab.~\ref{tab:sidd}, the results indicates the adaotivity of our method to real-world color image denoising. Our method achieve better result that outperforms CBM3D\cite{dabov2007color} and MC-WNNM\cite{xu2017multi} by nearly 10dB. 

\subsection{Qualitative results} We compare the visual quality of our proposed method DnLUT with other methods in Fig.~\ref{fig:Gua} and Fig.~\ref{fig:sidd}. In the first row from LUT-based methods in Fig.~\ref{fig:Gua}, it shows severe color distortion in these cases, while our method achieves similar visual quality as computation-heavy methods like DnCNN and CBM3D. In Fig.~\ref{fig:sidd}, results from both LUT-based and classical methods suffer from color distortion and contain over-smooth areas. On the contrary, our method maintains the color consistency and restored more details.


\begin{table*}[htp]
    \centering
    \caption{Efficiency evaluation of three categories color image denoising methods. We use the Qualcomm Snapdragon 8 Gen 2 as the mobile platform. The energy cost is calculated on the $512 \times 512$ resolution color images.}
    %Note that the latency of interpolation in GPU is approaching to 0, so we do not indicate it in the table.    &  &  &  
    \begin{tabular}
    {p{15mm}<{\centering}  p{28mm}<{\centering} p{20mm}<{\centering}  p{25mm}<{\centering}  p{25mm}<{\centering}  p{15mm}<{\centering}  p{20mm}<{\centering}}
    % {cccccc}
    \toprule[1.1pt]
      % \hline
      &Method & Platform &Runtime(ms) $256\times256$& Runtime(ms) $512\times512$ &Energy Cost (pJ) & Storage (KB) \\
      \hline
       \multirow{5}{*}{LUT} &SR-LUT\cite{jo2021practical} &Mobile &  6 & 19 &149.98M & 82\\
        &MuLUT\cite{li2022mulut} & Mobile &  21 & 80 & 899.88M & 489\\
        &RC-LUT\cite{gharbi2017deep} & Mobile &  18 & 78 & 612.92M & 326\\
        &SPF-LUT\cite{li2024look} & Mobile& 72 & 257 & 2.32G &30,178 \\
        &DnLUT(ours) & Mobile & 23  & 88 & 687.34M & 518\\
        \midrule
        \multirow{2}{*}{Classical}&CBM3D\cite{zhang2022clut} & PC & 3,189 & 14,343& 4.82G & -\\
        &MC-WNNM\cite{xu2017multi}  & PC & 74,290 & 293,424  & 89.23G & -\\
        \midrule
        \multirow{2}{*}{DNN}&DnCNN\cite{zhang2017beyond} & Mobile & 543 & 1,923 &542.53G & 2,239\\
        &SwinIR\cite{liang2021swinir} & Mobile & 73,234 & 274,453&12.03T & 45,499\\
      % \hline
      \bottomrule[1.1pt]
      
    \end{tabular}
    

    \label{tab:burden}
    % \vspace{-1em}
\end{table*}

\subsection{Efficiency Evaluation}
We conduct efficiency evaluation for different kinds of methods in terms of theoretical energy cost, runtime, and storage occupation in Tab.~\ref{tab:burden}. 

\noindent \textbf{Energy cost.} Following AdderSR\cite{song2021addersr}, we calculate the statistics of multiplications and additions in different data types required
by each method and estimate their total energy cost. Our method saves $70\%$ energy cost of SPF-LUT but with a gain of above 1dB in cPSNR. Besides, while classical or DNN-based methods achieve better results, they still need large computation which is inaccessible in edge devices. \eg, DnCNN need nearly $\times 800$ more energy compared to DnLUT.

\noindent \textbf{Runtime.} The applicatiton of LUT-based methods, which is based on the standard JAVA API, are implemented on the ANDROID platform. DnLUT maintains the nature of fast inference speed of SR-LUT\cite{jo2021practical}, showing a clear virtue compared with classical and DNN-based methods. Specifically, we use Pytorch-cpu for running DnCNN on the mobile platform and it consumes more than $20\times$ time. Additionally, DnLUT could be applied to specific devices with on-device optimization, such as FPGA, for even faster inference.

\noindent \textbf{Storage occupation.} DnLUT only need nearly 500 KB storage occupation which is much lower than the L2-cache in the widely used chips. It enables efficient lookup operations with simple dependencies.

\subsection{Effectiveness of Plug-in PCM}
Tab.~\ref{tab:pcm} show the cPSNR tested on 4 widely used synthetic validation datasets with Gaussian noise level $\sigma = 25$ and 2 real-world validation datasets of existing methods w./w.o. PCM module. PCM is not limited to a specific LUT method. By incorporating PCM, all LUT-based methods have shown significant performance improvements across various datasets. As shown in Fig.~\ref{fig:PCM}, the color distortion in the smooth area is attenuated, leading to a better perceptual quality.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figure/PCM.pdf}
    \caption{Visualization of LUT-based method with plug-in PCM.}
    \label{fig:PCM}
\end{figure}

\subsection{Ablation study}
Next, we use the Gaussian color image denoising benchmark for ablation studies to verify the critical components in DnLUT.

\subsubsection{Channel-spatial-wise convolution}
Channel indexing, as introduced in \cite{zamir2021multi}, is a channel-wise kernel with a $1\times1$
1×1 receptive field (RF) designed to extract RGB channel information. This design allows it to be converted into a 3D LUT during inference. We conducted experiments using various combinations of channel-wise, spatial-wise, and our proposed channel-spatial-wise kernels. For simplicity, our implementation employs a single channel indexing module, two stacked L-shaped convolution modules, and one PCM as the foundational components.
As evidenced in Tab.~\ref{tab:indexing}, a naive combination of channel-wise and spatial-wise convolutions results in inferior performance. An alternative approach, which involves solely applying channel-spatial-wise convolution, is constrained by its limited RF and struggles to effectively attenuate noise in smooth areas. However, incorporating both spatial-wise and channel-spatial-wise convolutions leads to a substantial performance improvement. Given that the channel-spatial-wise convolution already captures the full color information, the inclusion of channel-wise convolution offers only minimal additional benefits.
\subsubsection{L-shaped convolution}
To further verify the effectiveness of our proposed L-shaped convolution, we substitute all the L-shaped convolution with a normal $2\times2$ spatial-wise kernel, denoted as S in Tab.~\ref{tab:l}. While the normal kernel bring minimal improvement, our proposed L-shaped convolution could be converted to a 3D LUT, saving $17\times$ storage occupation that paves the way for stacking spatial-wise convolution. 
\begin{table}[htp]
    \centering
    \caption{Different combinations of channel-wise, spatial-wise, and our channel-spatial-wise kernels. These kernels are represented by channel indexing\cite{li2024toward}, L-shaped kernel, and PCM. The table presents cPSNR(dB) values.}

    \begin{tabular}{p{15mm}<{\centering}  p{15mm}<{\centering}  p{25mm}<{\centering}  p{12mm}<{\centering}  }
        \toprule[1.1pt]
        Channel & Spatial & Channel-spatial &CBSD68 \\
        \hline
        & \checkmark & & 29.77\\
        & & \checkmark & 30.15\\
        \checkmark & \checkmark & & 30.21\\
        & \checkmark & \checkmark & 31.41\\
        \checkmark & \checkmark& \checkmark & 31.47\\
        \bottomrule[1.1pt]
        % \vspace{-1.0em}
        
    \end{tabular}
    \label{tab:indexing}
\end{table}

\begin{table}[htp]
    \centering
    \caption{Comparison of L-shaped kernel and $2\times2$ spatial-wise kernel. The table presents cPSNR(dB) values.}
    \begin{tabular}{ccccc}
        \toprule[1.1pt]
      % \hline
       Method& CBSD68 & Kodak&McMaster & LUT Size(KB) \\
            \hline
        PCM+L  & 29.88 & 30.24 &30.44 &494\textcolor{red}{+24}\\
        PCM+S  & 29.91 & 30.32 & 30.48&494\textcolor{red}{+408}\\
      % \hline
      \bottomrule[1.1pt]
      \vspace{-2.0em}
    \end{tabular}
    \label{tab:l}
\end{table}



% \setlength{\parskip}{-1em}

% \subsubsection{Channel L-shape convolution}

==> sec/5_conclusion_bak.tex <==
% \setlength{\parskip}{-1em}
%\section{Discussion}
%\noindent \textbf{Energy cost.} The energy cost of DnLUT comes from the interpolation for correct the distortion during the sampled indexing.

\section{Conclusion}
This work has proposed the LUT-based color image denoising method, DnLUT, for extremely low-cost and high-speed color image denoising. We reveal that exsiting LUT-based methods are based on spatial-wise LUTs which lack of channel-spatial correlations for color image denoising. To this end, a novel pairwise channel mixer is devised to effectively build this connection with uncompromising storage occupation. Throughout the development of DnLUT, we discover the redundancy of the rotational kernels comes from the overlapping pixels. Inspired by this insight, a L-shaped kernel is designed in DnLUT, converting the 4D LUT to 3D LUT during inference for saving $\times17$ storage occupation and still maintaining the performance. With the concerted efforts of these novel designs, our DnLUT outperform the state-of-the-art LUT-based method in color image denoising by over 1 dB, and reduces the cost to only $0.1\%$ of DnCNN.

